Adversarially Robust Learning Could Leverage Computational Hardness

Over recent years, devising classification algorithms that are robust to adversarial perturbations has emerged as a challenging problem. In particular, deep neural nets (DNNs) seem to be susceptible to small imperceptible changes over test instances. However, the line of work in provable robustness, so far, has been focused on information-theoretic robustness, ruling out even the existence of any adversarial examples. In this work, we study whether there is a hope to benefit from algorithmic nature of an attacker that searches for adversarial examples, and ask whether there is any learning task for which it is possible to design classifiers that are only robust against polynomial-time adversaries. Indeed, numerous cryptographic tasks can only be secure against computationally bounded adversaries, and are indeed impossible for computationally unbounded attackers. Thus, it is natural to ask if the same strategy could help robust learning. We show that computational limitation of attackers can indeed be useful in robust learning by demonstrating the possibility of a classifier for some learning task for which computational and information theoretic adversaries of bounded perturbations have very different power. Namely, while computationally unbounded adversaries can attack successfully and find adversarial examples with small perturbation, polynomial time adversaries are unable to do so unless they can break standard cryptographic hardness assumptions. Our results, therefore, indicate that perhaps a similar approach to cryptography (relying on computational hardness) holds promise for achieving computationally robust machine learning. On the reverse directions, we also show that the existence of such learning task in which computational robustness beats information theoretic robustness requires computational hardness by implying (average-case) hardness of NP.

==> preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{nicefrac}
\usepackage{xspace}
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
\usepackage{times}
\usepackage{color}

%\usepackage[margin=1.2in]{geometry}
%\usepackage{times}
% \usepackage{xfrac}

%\include{definitions}
%\usepackage[useregional,showseconds=false]{datetime2}

\usepackage{paralist} % needed for asparaitem for both normal article class and the NIPS specific template
\usepackage{psfrag}
\usepackage{dsfont}
\usepackage{paralist}


\definecolor{RoyalBlue}{cmyk}{1, 0.50, 0, 0}
\definecolor{ForestGreen}{cmyk}{0.864, 0.0, 0.429, 0.396}
\definecolor{Brown}{cmyk}{0.0,0.692,0.925,0.529}

\usepackage{todonotes}


%\usepackage[numbers,square,sort&compress]{natbib}
%\newcommand{\shortcite}[1]{\citep{#1}}

%% \usepackage[usenames]{color}
%% \usepackage{hyperref}



\usepackage[english, ruled, linesnumbered, vlined]{algorithm2e}

\usepackage{amssymb,amsmath,amsthm}
%\usepackage{txfonts}

\usepackage{subfigure}
\usepackage[makeroom]{cancel}
\usepackage{thmtools,thm-restate}
%\usepackage{upgreek}
\usepackage{comment}
\usepackage{multirow}


\input{macros}

% Latex notation used by Xiao
\newcommand{\shortsection}[1]{\vspace*{1ex}\noindent{\bf #1.}}
\definecolor{carnelian}{rgb}{0.7, 0.11, 0.11}
\newcommand{\Xnote}[1]{{\ifcomments\color{carnelian} [\bf {X:}  #1]}\fi}


\def \db {\mathbf{d}}
\def \bx {\bm{x}}
\def \bc {\bm{c}}
\def \bb {\bm{b}}
\def \bu {\bm{u}}
\def \br {\bm{r}}
\def \bA {\bm{A}}
\def \tbx {\tilde{\bx}}

\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\ind}{\mathds{1}}

%\def \AdvRisk {\text{AdvRisk}}
\def \init {\text{init}}
\def \exp {\text{exp}}
%\title{\mypapertitle}
%\author{\mypaperauthors}


%################################################


\usepackage{todonotes}
\newcommand{\ifcomments}{\iffalse}


\newcommand{\MohNote}[1]{\ifcomments{\color{red} [{\bf Mohammad:}  #1]}\fi}
\newcommand{\Mnote}[1]{\MohNote{#1}}
\newcommand{\sanjam}[1]{\ifcomments{\color{red} [{\bf Sanjam:}  #1]}\fi}
\newcommand{\Snote}[1]{\ifcomments{\color{red} [{\bf Saeed:}  #1]}\fi}
\newcommand{\SomeshNote}[1]{{\ifcomments\color{ForestGreen} [\bf {Somesh:}  #1]}\fi}



%\usepackage[numbers,square,sort&compress]{natbib}
%\newcommand{\shortcite}[1]{\citep{#1}}

%% \usepackage[usenames]{color}
%% \usepackage{hyperref}

%\usepackage[english, ruled, linesnumbered, vlined]{algorithm2e}


